Sampling From Autoencoders' Latent Space via Quantization And Probability Mass Function Concepts

In this study, we focus on sampling from the latent space of generative models built upon autoencoders so as the reconstructed samples are lifelike images. To do to, we introduce a novel post-training sampling algorithm rooted in the concept of probability mass functions, coupled with a quantization process. Our proposed algorithm establishes a vicinity around each latent vector from the input data and then proceeds to draw samples from these defined neighborhoods. This strategic approach ensures that the sampled latent vectors predominantly inhabit high-probability regions, which, in turn, can be effectively transformed into authentic real-world images. A noteworthy point of comparison for our sampling algorithm is the sampling technique based on Gaussian mixture models (GMM), owing to its inherent capability to represent clusters. Remarkably, we manage to improve the time complexity from the previous $\mathcal{O}(n\times d \times k \times i)$ associated with GMM sampling to a much more streamlined $\mathcal{O}(n\times d)$, thereby resulting in substantial speedup during runtime. Moreover, our experimental results, gauged through the Fr\'echet inception distance (FID) for image generation, underscore the superior performance of our sampling algorithm across a diverse range of models and datasets. On the MNIST benchmark dataset, our approach outperforms GMM sampling by yielding a noteworthy improvement of up to $0.89$ in FID value. Furthermore, when it comes to generating images of faces and ocular images, our approach showcases substantial enhancements with FID improvements of $1.69$ and $0.87$ respectively, as compared to GMM sampling, as evidenced on the CelebA and MOBIUS datasets. Lastly, we substantiate our methodology's efficacy in estimating latent space distributions in contrast to GMM sampling, particularly through the lens of the Wasserstein distance.

==> files/extras.tex <==
\begin{table}[htb]
    \centering
    \caption{Comparison of Gaussian Mixture Model (GMM) sampling to Probability Mass Function (PMF) sampling in terms of FID and Wasserstein distance on the MNIST, CIFAR-10 and CelebA data sets. The columns \#dist and $k$ represents the number of distributions used in the GMM sampling and the number of partitions per dimension in the PMF sampling method, minimizing the FID metric, respectively.}
    \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{cccccccc}
    \toprule
         & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{GMM}} & \multicolumn{3}{c}{\textbf{PMF}}  \\
         &  & FID & $\mathcal{W}_2$ & \#dists & FID & $\mathcal{W}_2$ & $k$  \\
        \midrule
        \multirow{5}{*}{\rotatebox[origin=c]{90}{MNIST}} & AE & \phantom{0}4.66 & 905.13 & 20 & \textbf{\phantom{0}4.19} & \textbf{832.52} & \phantom{0}8 \\
        & VAE & \phantom{0}8.66 & \textbf{13.69} & 12 & \textbf{\phantom{0}8.57} & 14.26 & 10\\
        & $\beta$-VAE & 11.98 & \textbf{13.50} & 12 & \textbf{11.74} & 53.82 & \phantom{0}2\\
        & WAE & \phantom{0}4.67 & 940.01 & 18 & \textbf{\phantom{0}4.24} & \textbf{859.72} & \phantom{0}8\\
        & InfoVAE & \phantom{0}8.84 & \textbf{13.01} & 10 & \textbf{\phantom{0}7.95} & 49.28 & \phantom{0}2\\\midrule
        
         \multirow{5}{*}{\rotatebox[origin=c]{90}{CIFAR-10}} & AE & 10.67 & 345.74 & 12 & \textbf{\phantom{0}9.72} & 348.95 & 20 \\
        & VAE & 14.03 & 88.67 & 18 & \textbf{13.89} & 119.91 & \phantom{0}4\\
        & $\beta$-VAE & 15.27 & 88.58 & \phantom{0}4 & \textbf{14.99} & 294.58 & \phantom{0}2 \\
        & WAE & 10.63 & 336.23 & 10 & \textbf{\phantom{0}9.72} & 370.30 & 16\\
        & InfoVAE & 14.11 & 86.21 & \phantom{0}6 & \textbf{13.75} & 297.28 & \phantom{0}2\\\midrule
        
         \multirow{5}{*}{\rotatebox[origin=c]{90}{CelebA}} & AE & 10.63 & $4.6 \times 10^{5}$ & 8 & \textbf{\phantom{0}8.94} & $4.3 \times 10^{5}$ & 20 \\
        & VAE & 10.49 & 192.96 & 16 & \textbf{\phantom{0}9.25} & 196.34 & 14 \\
        & $\beta$-VAE & 11.10 & 197.18 & 20 & \textbf{\phantom{0}9.91} & 198.25 & 20 \\
        & WAE & 10.58 & $\mathbf{4.9 \times 10^{5}}$ & 20 & \textbf{\phantom{0}8.89} & $4.8 \times 10^{5}$ & 12 \\
        & InfoVAE & 10.56 & 196.85 & 20 & \textbf{\phantom{0}9.33} & 198.47 & 12 \\\bottomrule
    \end{tabular}
    }
    \label{tab:fid_results}
\end{table}

\section{Network architectures}
\label{archis}
\subsection{MNIST data set}
\begin{minted}{python}
import torch 
import numpy as np

class Encoder(pl.Lig HningModule):
    def __init__(self, latent_dim=64):
        super().__init__()
        self.encoder = torch.nn.Sequential(
            torch.nn.Conv2d(1, 128, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(128),
            torch.nn.ReLU(),
            torch.nn.Conv2d(128, 256, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(256),
            torch.nn.ReLU(),
            torch.nn.Conv2d(256, 512, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(512),
            torch.nn.ReLU(),
            torch.nn.Conv2d(512, 1024, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(1024),
            torch.nn.ReLU(),
            flatten())
        self.mu = torch.nn.Linear(1024, latent_dim)
        self.logvar = torch.nn.Linear(1024, latent_dim)

    def forward(self, x):
        encodings = self.encoder(x)
        return self.mu(encodings), self.logvar(encodings)

class Decoder(pl.Lig HningModule):
    def __init__(self, latent_dim=64, shape=(1024, 4, 4)):
        super().__init__()
        self.shape = shape
        self.decoder = torch.nn.Sequential(
            torch.nn.Linear(latent_dim, 1024*4*4),
            unflatten(shape),
            torch.nn.ConvTranspose2d(1024, 512, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(512),
            torch.nn.ReLU(),
            torch.nn.ConvTranspose2d(512, 256, kernel_size=4, stride=2, padding=2),
            torch.nn.BatchNorm2d(256),
            torch.nn.ReLU(),
            torch.nn.ConvTranspose2d(256, 1, kernel_size=4, stride=2, padding=1),
            torch.nn.Sigmoid())
    
    def forward(self, z):
        return self.decoder(out)
\end{minted}

\subsection{CIFAR-10 data set}
\begin{minted}{python}
import torch 
import numpy as np

class Encoder(pl.Lig HningModule):
    def __init__(self, latent_dim=64):
        super().__init__()
        self.encoder = torch.nn.Sequential(
            torch.nn.Conv2d(3, 128, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(128),
            torch.nn.ReLU(),
            torch.nn.Conv2d(128, 256, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(256),
            torch.nn.ReLU(),
            torch.nn.Conv2d(256, 512, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(512),
            torch.nn.ReLU(),
            torch.nn.Conv2d(512, 1024, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(1024),
            torch.nn.ReLU(),
            flatten()
        )

        self.mu = torch.nn.Linear(1024*2*2, latent_dim)
        self.logvar = torch.nn.Linear(1024*2*2, latent_dim)

    def forward(self, x):
        encodings = self.encoder(x)
        return self.mu(encodings), self.logvar(encodings)
        
class Decoder(pl.Lig HningModule):
    def __init__(self, latent_dim=64, shape=(1024, 4, 4)):
        super().__init__()
        self.shape = shape
        self.decoder = torch.nn.Sequential(
            torch.nn.Linear(latent_dim, 1024*4*4),
            unflatten(shape),
            torch.nn.ConvTranspose2d(1024, 512, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(512),
            torch.nn.ReLU(),
            torch.nn.ConvTranspose2d(512, 256, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(256),
            torch.nn.ReLU(),
            torch.nn.ConvTranspose2d(256, 3, kernel_size=4, stride=2, padding=1),
            torch.nn.Sigmoid()
        )
    
    def forward(self, z):
        return self.decoder(z)
\end{minted}

\subsection{CelebA data set}
\begin{minted}{python}
import torch 
import numpy as np

class Encoder(pl.LighningModule):
    def __init__(self, latent_dim=64):
        super().__init__()
        self.encoder = torch.nn.Sequential(
            torch.nn.Conv2d(3, 128, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(128),
            torch.nn.ReLU(),
            torch.nn.Conv2d(128, 256, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(256),
            torch.nn.ReLU(),
            torch.nn.Conv2d(256, 512, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(512),
            torch.nn.ReLU(),
            torch.nn.Conv2d(512, 1024, kernel_size=4, stride=2, padding=1),
            torch.nn.BatchNorm2d(1024),
            torch.nn.ReLU(),
            flatten()
        )

        self.mu = torch.nn.Linear(1024*13*11, latent_dim)
        self.logvar = torch.nn.Linear(1024*13*11, latent_dim)

    def forward(self, x):
        encodings = self.encoder(x)
        return self.mu(encodings), self.logvar(encodings)

class Decoder(pl.LighningModule):
    def __init__(self, latent_dim=64, shape=(1024, 13, 11)):
        super().__init__()
        self.shape = shape
        self.decoder = torch.nn.Sequential(
            torch.nn.Linear(latent_dim, 1024*13*11),
            torch.nn.BatchNorm1d(1024*13*11),
            torch.nn.ReLU(),
            unflatten(shape),
            torch.nn.ConvTranspose2d(1024, 512, kernel_size=(3,4), stride=2, padding=(0,1)),
            torch.nn.BatchNorm2d(512),
            torch.nn.ReLU(),
            torch.nn.ConvTranspose2d(512, 256, kernel_size=(3,4), stride=2, padding=(0,1)),
            torch.nn.BatchNorm2d(256),
            torch.nn.ReLU(),
            torch.nn.ConvTranspose2d(256, 128, kernel_size=(3,4), stride=2, padding=1),
            torch.nn.BatchNorm2d(128),
            torch.nn.ReLU(),
            torch.nn.ConvTranspose2d(128, 3, kernel_size=(2,4), stride=2, padding=0),
            torch.nn.Sigmoid()
        )
    
    def forward(self, z):
        return self.decoder(z)
\end{minted}


\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|cc|c|c|c|c|c|}
    \toprule
        Data set & & AE & VAE & $\beta$-VAE & WAE & InfoVAE \\\midrule
        \multirow{2}{*}{MNIST} & $\mu$ & \phantom{0}869.22 & 100.00 & \phantom{0}99.82 & 881.99 & 98.06 \\
        & $\sigma$ & \phantom{0}278.99 & \phantom{00}3.69 & \phantom{00}3.24 & 277.05 & \phantom{0}5.12 \\ \midrule
        \multirow{2}{*}{CIFAR-10} & $\mu$ & \phantom{0}204.17 & \phantom{0}99.90 & \phantom{0}99.92 & 207.06 & 98.67 \\
        & $\sigma$ & \phantom{00}92.56 & \phantom{00}6.16 & \phantom{00}5.93 & \phantom{0}94.70 & \phantom{0}6.49 \\ \midrule
        \multirow{2}{*}{CelebA} & $\mu$ & 6964.68 & 139.11 & 140.32 & 7148.37 & 138.95 \\
        & $\sigma$ & 4409.65 & \phantom{0}20.91 & \phantom{0}16.18 & 3663.28 & \phantom{0}21.09 \\ \midrule
        \multirow{2}{*}{MOBIUS} & $\mu$ & \\
        & $\sigma$ \\ \midrule
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:singular values}
\end{table}
